Distributed Algorithm for Matching between Individuals and Activities

In this paper, we introduce an agent-based model for coalition formation which is suitable for our usecase. We propose here two clearing-houses mechanisms that return sound matchings. The first aims at maximizing the global satisfaction of the individuals. The second ensures that all individuals are assigned as much as possible to a preferred activity. Our experiments show that the outcome of our algorithms are better than those obtained with the classical search/optimization techniques. Moreover, their distribution speeds up their runtime.

==> figures/dilemma.tex <==
\node (i11) {\inditwo}; 
\node (i12) [right of=i11] {\indione};
\node (pref11) [right of=i12] {\prefI{blue}{1}};
\node (i13) [right of=pref11] {\indione}; 
\node (pref12) [right of=i13] {\prefI{blue}{1}}; 
\node (i14) [right of=pref12] {\indithree};
\node (i15) [right of=i14] {\indione};
\node (pref13) [right of=i15] {\prefI{blue}{1}};
\node (i16) [right of=pref13] {\indifour}; 
\node (i17) [right of=i16] {\indione}; 

\node (i21) [below =.2cm of i11] {\indione}; 
\node (i22) [right of=i21] {\inditwo};
\node (pref21) [right of=i22] {\prefI{cyan}{2}};
\node (i23) [right of=pref21] {\indithree}; 
\node (i24) [right of=i23] {\inditwo}; 
\node (pref22) [right of=i24] {\prefI{cyan}{2}}; 
\node (i25) [right of=pref22] {\inditwo};
\node (pref23) [right of=i25] {\prefI{cyan}{2}};
\node (i26) [right of=pref23] {\indifour}; 
\node (i27) [right of=i26] {\inditwo}; 

\node (i31) [below =.2cm of i21] {\indione}; 
\node (i32) [right of=i31] {\indithree};
\node (pref31) [right of=i32] {\prefI{magenta}{3}};
\node (i33) [right of=pref31] {\inditwo}; 
\node (i34) [right of=i33] {\indithree}; 
\node (pref32) [right of=i34] {\prefI{magenta}{3}}; 
\node (i35) [right of=pref32] {\indithree};
\node (pref33) [right of=i35] {\prefI{magenta}{3}};
\node (i36) [right of=pref33] {\indifour};
\node (i37) [right of=i36] {\indithree}; 

\node (i41) [below =.2cm of i31] {\indione}; 
\node (i42) [right of=i41] {\indifour};
\node (pref41) [right of=i42] {\equivI{red}{4}};
\node (i43) [right of=pref41] {\inditwo}; 
\node (i44) [right of=i43] {\indifour}; 
\node (pref42) [right of=i44] {\prefI{red}{4}}; 
\node (i45) [right of=pref42] {\indifour};
\node (pref43) [right of=i45] {\prefI{red}{4}};
\node (i46) [right of=pref43] {\indithree};
\node (i47) [right of=i46] {\indifour}; 



==> figures/traceInclusiveSolverEgalitarian.tex <==
\begin{minted}[xleftmargin=20 pt,linenos=true,mathescape=true,escapeinside=||,mathescape=true,fontsize=\footnotesize]{text}
a(2): [] b(2): [] |$\theta$|: [1, 2, 3, 4]
4 selects a with []
Since a is not full, 
4 is assigned to a
\end{minted}

\begin{minted}[xleftmargin=20 pt,linenos=true,mathescape=true,escapeinside=||,fontsize=\footnotesize,firstnumber=last]{text}
a(2): [4] b(2): [] |$\theta$|: [1, 2, 3]
3 selects a with [4]
Since a is not full, 
3 is assigned to a
\end{minted}

\begin{minted}[xleftmargin=20 pt,linenos=true,mathescape=true,escapeinside=||,fontsize=\footnotesize,firstnumber=last]{text}
a(2): [3, 4] b(2): [] |$\theta$|: [1, 2]
2 selects a with [3, 4]
[4, 3].umin(a)=0,083
[4, 2].umin(a)=0,083
[3, 2].umin(a)=0,333
Since [3, 2] is selected,
4 is excluded from a
2 is assigned to a
\end{minted}

\begin{minted}[xleftmargin=20 pt,linenos=true,mathescape=true,escapeinside=||,fontsize=\footnotesize,firstnumber=last]{text}
a(2): [2, 3] b(2): [] |$\theta$|: [1, 4]
1 selects a with [2, 3]
[3, 2].umin(a)=0,333
[3, 1].umin(a)=0,167
[2, 1].umin(a)=0,417
Since [2, 1] is selected,
3 is excluded from a
1 is assigned to a
\end{minted}


\begin{minted}[xleftmargin=20 pt,linenos=true,mathescape=true,escapeinside=||,fontsize=\footnotesize,firstnumber=last]{text}
a(2): [1, 2] b(2): [3] |$\theta$|: [4]
4 selects b with [3]
Since b is not full, 
4 is assigned to b
\end{minted}

\begin{minted}[xleftmargin=20 pt,linenos=true,mathescape=true,escapeinside=||,fontsize=\footnotesize,firstnumber=last]{text}
a(2): [1, 2] b(2): [3, 4] |$\theta$|: []
\end{minted}









==> figures/traceMNSolverExactUtil.tex <==
\begin{minted}[xleftmargin=20 pt,linenos=true,mathescape=true,escapeinside=||,fontsize=\footnotesize]{text}
M: a(2): [] b(2): [] |$\theta$|: [1, 2, 3, 4]
Since a is free,
4 is assigned to a
\end{minted}

\begin{minted}[xleftmargin=20 pt,linenos=true,mathescape=true,escapeinside=||,fontsize=\footnotesize,firstnumber=last]{text}
M: a(2): [4] b(2): [] |$\theta$|: [1, 2, 3]
3 selects a with [4]
[3].usum(a)=0,250
[4].usum(a)=0,250
[4, 3].usum(a)=0,167
Since [3] is selected,
4 is excluded from a
3 is assigned to a
\end{minted}

\begin{minted}[xleftmargin=20 pt,linenos=true,mathescape=true,escapeinside=||,fontsize=\footnotesize,firstnumber=last]{text}
M: a(2): [3] b(2): [] |$\theta$|: [1, 2, 4]
2 selects a with [3]
[2].usum(a)=0,250
[3].usum(a)=0,250
[3, 2].usum(a)=0,667
Since [3, 2] is selected,
2 is assigned to a
\end{minted}

\begin{minted}[xleftmargin=20 pt,linenos=true,mathescape=true,escapeinside=||,fontsize=\footnotesize,firstnumber=last]{text}
M: a(2): [2, 3] b(2): [] |$\theta$|: [1, 4]
1 selects a with [2, 3]
[3, 2].usum(a)=0,667
[1].usums(a)=0,250
[3].usum(a)=0,250
[2, 1].usum(a)=0,833
[2].usum(a)=0,250
[3, 1].usum(a)=0,583
Since [2, 1] is selected,
3 is excluded from a
1 is assigned to a
\end{minted}


\begin{minted}[xleftmargin=20 pt,linenos=true,mathescape=true,escapeinside=||,fontsize=\footnotesize,firstnumber=last]{text}
M: a(2): [1, 2] b(2): [] |$\theta$|: [3, 4]
Since b is free, 
3 is assigned to b
\end{minted}

\begin{minted}[xleftmargin=20 pt,linenos=true,mathescape=true,escapeinside=||,fontsize=\footnotesize,firstnumber=last]{text}
M: a(2): [1, 2] b(2): [3] |$\theta$|: [4]
4 selects b with [3]
[4].usum(b)=0,125
[3].usum(b)=0,125
[3, 4].usum(b)=-0,083
Since [4] is selected,
3 is excluded from b
4 is assigned to b
\end{minted}

\begin{minted}[xleftmargin=20 pt,linenos=true,mathescape=true,escapeinside=||,fontsize=\footnotesize,firstnumber=last]{text}
M: a(2): [1, 2] b(2): [4] |$\theta$|: [3]
3 is definitely inactive
\end{minted}

\begin{minted}[xleftmargin=20 pt,linenos=true,mathescape=true,escapeinside=||,fontsize=\footnotesize,firstnumber=last]{text}
M: a(2): [1, 2] b(2): [4] |$\theta$|: [3]
\end{minted}

